CholecTriplet2021: A benchmark challenge for surgical action triplet recognition

Context-aware decision support in the operating room can foster surgical safety and efficiency by leveraging real-time feedback from surgical workflow analysis. Most existing works recognize surgical activities at a coarse-grained level, such as phases, steps or events, leaving out fine-grained interaction details about the surgical activity; yet those are needed for more helpful AI assistance in the operating room. Recognizing surgical actions as triplets of <instrument, verb, target> combination delivers comprehensive details about the activities taking place in surgical videos. This paper presents CholecTriplet2021: an endoscopic vision challenge organized at MICCAI 2021 for the recognition of surgical action triplets in laparoscopic videos. The challenge granted private access to the large-scale CholecT50 dataset, which is annotated with action triplet information. In this paper, we present the challenge setup and assessment of the state-of-the-art deep learning methods proposed by the participants during the challenge. A total of 4 baseline methods from the challenge organizers and 19 new deep learning algorithms by competing teams are presented to recognize surgical action triplets directly from surgical videos, achieving mean average precision (mAP) ranging from 4.2% to 38.1%. This study also analyzes the significance of the results obtained by the presented approaches, performs a thorough methodological comparison between them, in-depth result analysis, and proposes a novel ensemble method for enhanced recognition. Our analysis shows that surgical workflow analysis is not yet solved, and also highlights interesting directions for future research on fine-grained surgical activity recognition which is of utmost importance for the development of AI in surgery.

==> highlights.tex <==


1. A critical study on surgical action triplet recognition in form a deep learning challenge.

2. A summary of deep learning methods presented at the challenge.

3. An in-depth methodological comparative analysis, providing a comprehensive overview of possible strategies for tackling the surgical action triplet problem.

4. Simple but effective ensemble algorithms setting a new baseline with an improvement of +4.3\% AP to the challenge methods for the surgical action triplet recognition.

5. An in-depth quantitative and qualitative result analysis considering multiple metrics to cover all aspects of the triplet recognition problem.



% \newpage
\onecolumn
\section*{Highlights}


\begin{enumerate}
    \item A comprehensive study on surgical action triplet recognition directly from videos.
    \item A new attention mechanism that is guided by weakly-supervised class activation maps for more precise detection.
    \item A Transformer-inspired neural network that utilizes self- and cross-attention {\red mechanisms} for action triplet recognition.
    \item Introduction of CholecT50, a large endoscopic dataset for action triplet recognition.
    \item Extensive comparison and ablation study showing state-of-the-art results and discussion of clinical relevance.
\end{enumerate}

\thispagestyle{empty}


\newpage
\section*{Suggested Editors}
\begin{enumerate}
    \item \textbf{Kensaku Mori}\\ Nagoya University Graduate School of Engineering Department of Chrystalline Materials Science, Nagoya, Japan
    \item \textbf{Jocelyne Troccaz}\\Techniques for Biomedical Engineering and Complexity Management Informatics Mathematics and Applications Grenoble Laboratory, La Tronche cedex, France
    \item \textbf{Tom Vercauteren} \\ King's College London, London, United Kingdom
    
    
\end{enumerate}



\newpage
\section*{Suggested Reviewers}
\begin{enumerate}
    
    
\item 
\textbf{Name}: Prof. Raphael Sznitman \\
\textbf{Institution}: ARTORG Center, University of Bern\\
\textbf{Country}: Switzerland\\
\textbf{E-Mail}:  raphael.sznitman@artorg.unibe.ch\\
\textbf{Reason for the choice}: The professor leds a research in computational vision, probabilistic methods and statistical learning, applied to applications in Ophthalmology and biomedical imaging. He has multiple publications that use deep learning method for the modeling of surgical activities. Thus, he will provide an in-depth review of the submitted work.



\item 
\textbf{Name}: Dr. Max Allan \\
\textbf{Institution}: Intuitive Surgical, Inc\\
\textbf{Country}: United State of America\\
\textbf{E-Mail}: max.allan@intusurg.com\\
\textbf{Reason for the choice}: Max Allan is a researcher with both academic and industrial experience. He work on applying Computer Vision and Machine Learning to the da Vinci surgical robot and has multiple publications on surgical tool detection and activity recognition in Minimally Invasive Surgery.



\item 
\textbf{Name}: Darko Katic\\
\textbf{Institution}: Karlsruhe Institute of Technology\\
\textbf{Country}: Germany\\
\textbf{E-Mail}: darko.katic@kit.edu\\
\textbf{Reason for the choice}: He is a pioneer researcher on fine-grained surgical action recognition. In fact, his paper is one of the first that describe surgical actions as triplets of instrument, verb, and target. He is a prominent researcher in the computer-assisted intervention. Very easy to find on Google scholar on the topic in the manuscipt.

\end{enumerate}





